Astronomy potential of KM3NeT/ARCA

The KM3NeT/ARCA neutrino detector is currently under construction at 3500 m depth offshore Capo Passero, Sicily, in the Mediterranean Sea. The main science objectives are the detection of high-energy cosmic neutrinos and the discovery of their sources. Simulations were conducted for the full KM3NeT/ARCA detector, instrumenting a volume of 1 km$^3$, to estimate the sensitivity and discovery potential to point-like neutrino sources and an all-sky diffuse neutrino flux. This paper covers the reconstruction of track- and shower-like signatures, as well as the criteria employed for neutrino event selection. By leveraging both the track and shower observation channels, the KM3NeT/ARCA detector demonstrates the capability to detect the diffuse astrophysical neutrino flux within half a year of operation, achieving a 5$\sigma$ statistical significance. With an angular resolution below 0.1$^\circ$ for tracks and under 2$^\circ$ for showers, the sensitivity to point-like neutrino sources surpasses existing observed limits across the entire sky.

==> acknow.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Acknowledgements} The authors acknowledge the financial support of the funding agencies:
%Czeck
Czech Science Foundation (GA\u CR 24-12702S);
%France
Agence Nationale de la Recherche (contract ANR-15-CE31-0020), Centre National de la Recherche Scientifique (CNRS), Commission Europ\'eenne (FEDER fund and Marie Curie Program), LabEx UnivEarthS (ANR-10-LABX-0023 and ANR-18-IDEX-0001), Paris \^Ile-de-France Region, France;
%Georgia
Shota Rustaveli National Science Foundation of Georgia (SRNSFG, FR-22-13708), Georgia;
%Greece
The General Secretariat of Research and Innovation (GSRI), Greece;
%Italy
Istituto Nazionale di Fisica Nucleare (INFN) and Ministero dell’Universit{\`a} e della Ricerca (MUR), through PRIN 2022 program (Grant PANTHEON 2022E2J4RK, Next Generation EU) and PON R\&I program (Avviso n. 424 del 28 febbraio 2018, Progetto PACK-PIR01 00021), Italy; A. De Benedittis, R. Del Burgo, W. Idrissi Ibnsalih, A. Nayerhoda, G. Papalashvili, I. C. Rea, S. Santanastaso, A. Simonelli have been supported by the Italian Ministero dell'Universit{\`a} e della Ricerca (MUR), Progetto CIR01 00021 (Avviso n. 2595 del 24 dicembre 2019);
%Morocco
Ministry of Higher Education, Scientific Research and Innovation, Morocco, and the Arab Fund for Economic and Social Development, Kuwait;
%The Netherlands
Nederlandse organisatie voor Wetenschappelijk Onderzoek (NWO), the Netherlands;
%Poland
The National Science Centre, Poland (2021/41/N/ST2/01177); The grant “AstroCeNT: Particle Astrophysics Science and Technology Centre”, carried out within the International Research Agendas programme of the Foundation for Polish Science financed by the European Union under the European Regional Development Fund;
%Romania
National Authority for Scientific Research (ANCS), Romania;
%Slovakia
Slovak Research and Development Agency under Contract No. APVV-22-0413; Ministry of Education, Research, Development and Youth of the Slovak Republic;
%Spain
MCIN for PID2021-124591NB-C41, -C42, -C43, funded by MCIN/AEI/10.13039/501100011033 and by "ERDF A way of making Europe", for ASFAE/2022/014, ASFAE/2022 /023, with funding from the EU NextGenerationEU (PRTR-C17.I01), Generalitat Valenciana, and for CSIC-INFRA23013, Generalitat Valenciana for PROMETEO /2020/019, for Grant AST22\_6.2 with funding from Consejer\'{\i}a de Universidad, Investigaci\'on e Innovaci\'on and Gobierno de Espa\~na and European Union - NextGenerationEU, for CIDEGENT/2018/034, /2019/043, /2020/049, /2021/23 and for GRISOLIAP/2021/192 and EU for MSC/101025085, Spain;
%UK
The European Union's Horizon 2020 Research and Innovation Programme (ChETEC-INFRA - Project no. \newline 101008324).



==> authors.tex <==

\author{
S.~Aiello\thanksref{a} \and
A.~Albert\thanksref{b,bc} \and
M.~Alshamsi\thanksref{d,c} \and
S. Alves Garre\thanksref{e} \and
Z.~Aly\thanksref{c} \and
A. Ambrosone\thanksref{g,f} \and
F.~Ameli\thanksref{h} \and
M.~Andre\thanksref{i} \and
E.~Androutsou\thanksref{j} \and
M.~Anguita\thanksref{k} \and
L.~Aphecetche\thanksref{l} \and
M. Ardid\thanksref{m} \and
S. Ardid\thanksref{m} \and
H.~Atmani\thanksref{n} \and
J.~Aublin\thanksref{o} \and
F.~Badaracco\thanksref{p} \and
L.~Bailly-Salins\thanksref{q} \and
Z. Barda\v{c}ov\'{a}\thanksref{s,r} \and
B.~Baret\thanksref{o} \and
A. Bariego-Quintana\thanksref{e} \and
A.~Baruzzi\thanksref{p} \and
S.~Basegmez~du~Pree\thanksref{t} \and
Y.~Becherini\thanksref{o} \and
M.~Bendahman\thanksref{n,o} \and
F.~Benfenati\thanksref{v,u} \and
M.~Benhassi\thanksref{w,f} \and
D.\,M.~Benoit\thanksref{x} \and
E.~Berbee\thanksref{t} \and
V.~Bertin\thanksref{c} \and
S.~Biagi\thanksref{y} \and
M.~Boettcher\thanksref{z} \and
D.~Bonanno\thanksref{y} \and
J.~Boumaaza\thanksref{n} \and
M.~Bouta\thanksref{aa} \and
M.~Bouwhuis\thanksref{t} \and
C.~Bozza\thanksref{ab,f} \and
R.\,M.~Bozza\thanksref{g,f} \and
H.Br\^{a}nza\c{s}\thanksref{ac} \and
F.~Bretaudeau\thanksref{l} \and
M.~Breuhaus\thanksref{c} \and
R.~Bruijn\thanksref{ad,t} \and
J.~Brunner\thanksref{c} \and
R.~Bruno\thanksref{a} \and
E.~Buis\thanksref{ae,t} \and
R.~Buompane\thanksref{w,f} \and
J.~Busto\thanksref{c} \and
B.~Caiffi\thanksref{p} \and
D.~Calvo\thanksref{e} \and
S.~Campion\thanksref{h,af} \and
A.~Capone\thanksref{h,af} \and
F.~Carenini\thanksref{v,u} \and
V.~Carretero\thanksref{e} \and
T.~Cartraud\thanksref{o} \and
P.~Castaldi\thanksref{ag,u} \and
V.~Cecchini\thanksref{e} \and
S.~Celli\thanksref{h,af} \and
L.~Cerisy\thanksref{c} \and
M.~Chabab\thanksref{ah} \and
M.~Chadolias\thanksref{ai} \and
A.~Chen\thanksref{aj} \and
S.~Cherubini\thanksref{ak,y} \and
T.~Chiarusi\thanksref{u} \and
M.~Circella\thanksref{al} \and
R.~Cocimano\thanksref{y} \and
J.\,A.\,B.~Coelho\thanksref{o} \and
A.~Coleiro\thanksref{o} \and
R.~Coniglione\thanksref{y} \and
P.~Coyle\thanksref{c} \and
A.~Creusot\thanksref{o} \and
G.~Cuttone\thanksref{y} \and
R.~Dallier\thanksref{l} \and
Y.~Darras\thanksref{ai} \and
A.~De~Benedittis\thanksref{f} \and
B.~De~Martino\thanksref{c} \and
V.~Decoene\thanksref{l} \and
R.~Del~Burgo\thanksref{f} \and
I.~Del~Rosso\thanksref{v,u} \and
L.\,S.~Di~Mauro\thanksref{y} \and
I.~Di~Palma\thanksref{h,af} \and
A.\,F.~D\'\i{}az\thanksref{k} \and
C.~Diaz\thanksref{k} \and
D.~Diego-Tortosa\thanksref{y} \and
C.~Distefano\thanksref{y} \and
A.~Domi\thanksref{ai} \and
C.~Donzaud\thanksref{o} \and
D.~Dornic\thanksref{c} \and
M.~D{\"o}rr\thanksref{am} \and
E.~Drakopoulou\thanksref{j} \and
D.~Drouhin\thanksref{b,bc} \and
J.-G. Ducoin\thanksref{c} \and
R. Dvornick\'{y}\thanksref{s} \and
T.~Eberl\thanksref{ai} \and
E. Eckerov\'{a}\thanksref{s,r} \and
A.~Eddymaoui\thanksref{n} \and
T.~van~Eeden\thanksref{t,e1} \and % Assuming \corref and \ead for corresponding author
M.~Eff\thanksref{o} \and
D.~van~Eijk\thanksref{t} \and
I.~El~Bojaddaini\thanksref{aa} \and
S.~El~Hedri\thanksref{o} \and
A.~Enzenh\"ofer\thanksref{c} \and
G.~Ferrara\thanksref{y} \and
M.~D.~Filipovi\'c\thanksref{an} \and
F.~Filippini\thanksref{v,u} \and
D.~Franciotti\thanksref{y} \and
L.\,A.~Fusco\thanksref{ab,f} \and
J.~Gabriel\thanksref{ao} \and
S.~Gagliardini\thanksref{h} \and
T.~Gal\thanksref{ai} \and
J.~Garc{\'\i}a~M{\'e}ndez\thanksref{m} \and
A.~Garcia~Soto\thanksref{e} \and
C.~Gatius~Oliver\thanksref{t} \and
N.~Gei{\ss}elbrecht\thanksref{ai} \and
H.~Ghaddari\thanksref{aa} \and
L.~Gialanella\thanksref{f,w} \and
B.\,K.~Gibson\thanksref{x} \and
E.~Giorgio\thanksref{y} \and
I.~Goos\thanksref{o} \and
P.~Goswami\thanksref{o} \and
D.~Goupilliere\thanksref{q} \and
S.\,R.~Gozzini\thanksref{e} \and
R.~Gracia\thanksref{ai} \and
K.~Graf\thanksref{ai} \and
C.~Guidi\thanksref{ap,p} \and
B.~Guillon\thanksref{q} \and
M.~Guti{\'e}rrez\thanksref{aq} \and
H.~van~Haren\thanksref{ar} \and
A.~Heijboer\thanksref{t} \and
A.~Hekalo\thanksref{am} \and
L.~Hennig\thanksref{ai} \and
J.\,J.~Hern{\'a}ndez-Rey\thanksref{e} \and
W.~Idrissi~Ibnsalih\thanksref{f} \and
G.~Illuminati\thanksref{u} \and
M.~de~Jong\thanksref{as,t} \and
P.~de~Jong\thanksref{ad,t} \and
B.\,J.~Jung\thanksref{t} \and
P.~Kalaczy\'nski\thanksref{at,bd} \and
O.~Kalekin\thanksref{ai} \and
U.\,F.~Katz\thanksref{ai} \and
G.~Kistauri\thanksref{av,au} \and
C.~Kopper\thanksref{ai} \and
A.~Kouchner\thanksref{aw,o} \and
V.~Kueviakoe\thanksref{t} \and
V.~Kulikovskiy\thanksref{p} \and
R.~Kvatadze\thanksref{av} \and
M.~Labalme\thanksref{q} \and
R.~Lahmann\thanksref{ai} \and
G.~Larosa\thanksref{y} \and
C.~Lastoria\thanksref{c} \and
A.~Lazo\thanksref{e} \and
S.~Le~Stum\thanksref{c} \and
G.~Lehaut\thanksref{q} \and
E.~Leonora\thanksref{a} \and
N.~Lessing\thanksref{e} \and
G.~Levi\thanksref{v,u} \and
M.~Lindsey~Clark\thanksref{o} \and
F.~Longhitano\thanksref{a} \and
F.~Magnani\thanksref{c} \and
J.~Majumdar\thanksref{t} \and
L.~Malerba\thanksref{p} \and
F.~Mamedov\thanksref{r} \and
J.~Ma\'nczak\thanksref{e} \and
A.~Manfreda\thanksref{f} \and
M.~Marconi\thanksref{ap,p} \and
A.~Margiotta\thanksref{v,u} \and
A.~Marinelli\thanksref{f,g} \and
C.~Markou\thanksref{j} \and
L.~Martin\thanksref{l} \and
J.\,A.~Mart{\'\i}nez-Mora\thanksref{m} \and
F.~Marzaioli\thanksref{w,f} \and
M.~Mastrodicasa\thanksref{af,h} \and
S.~Mastroianni\thanksref{f} \and
S.~Miccich{\`e}\thanksref{y} \and
G.~Miele\thanksref{g,f} \and
P.~Migliozzi\thanksref{f} \and
E.~Migneco\thanksref{y} \and
M.\,L.~Mitsou\thanksref{f} \and
C.\,M.~Mollo\thanksref{f} \and
L. Morales-Gallegos\thanksref{w,f} \and
M.~Morga\thanksref{al} \and
A.~Moussa\thanksref{aa} \and
I.~Mozun~Mateo\thanksref{ay,ax} \and
R.~Muller\thanksref{t} \and
M.\,R.~Musone\thanksref{f,w} \and
M.~Musumeci\thanksref{y} \and
S.~Navas\thanksref{aq} \and
A.~Nayerhoda\thanksref{al} \and
C.\,A.~Nicolau\thanksref{h} \and
B.~Nkosi\thanksref{aj} \and
B.~{\'O}~Fearraigh\thanksref{ad,t} \and
V.~Oliviero\thanksref{g,f} \and
A.~Orlando\thanksref{y} \and
E.~Oukacha\thanksref{o} \and
D.~Paesani\thanksref{y} \and
J.~Palacios~Gonz{\'a}lez\thanksref{e} \and
G.~Papalashvili\thanksref{al,au} \and
V.~Parisi\thanksref{ap,p} \and
E.J. Pastor Gomez\thanksref{e} \and
A.~M.~P{\u a}un\thanksref{ac} \and
G.\,E.~P\u{a}v\u{a}la\c{s}\thanksref{ac} \and
I.~Pelegris\thanksref{j} \and
S. Pe\~{n}a Mart\'inez\thanksref{o} \and
M.~Perrin-Terrin\thanksref{c} \and
J.~Perronnel\thanksref{q} \and
V.~Pestel\thanksref{ay} \and
R.~Pestes\thanksref{o} \and
P.~Piattelli\thanksref{y} \and
C.~Poir{\`e}\thanksref{ab,f} \and
V.~Popa\thanksref{ac} \and
T.~Pradier\thanksref{b} \and
J.~Prado\thanksref{e} \and
S.~Pulvirenti\thanksref{y} \and
C.A.~Quiroz-Rangel\thanksref{m} \and
U.~Rahaman\thanksref{e} \and
N.~Randazzo\thanksref{a} \and
R.~Randriatoamanana\thanksref{l} \and
S.~Razzaque\thanksref{az} \and
I.\,C.~Rea\thanksref{f} \and
D.~Real\thanksref{e} \and
G.~Riccobene\thanksref{y} \and
J.~Robinson\thanksref{z} \and
A.~Romanov\thanksref{ap,p} \and
A. \v{S}aina\thanksref{e} \and
F.~Salesa~Greus\thanksref{e} \and
D.\,F.\,E.~Samtleben\thanksref{as,t} \and
A.~S{\'a}nchez~Losa\thanksref{e,al} \and
S.~Sanfilippo\thanksref{y} \and
M.~Sanguineti\thanksref{ap,p} \and
C.~Santonastaso\thanksref{w,f} \and
D.~Santonocito\thanksref{y} \and
P.~Sapienza\thanksref{y} \and
J.~Schnabel\thanksref{ai} \and
J.~Schumann\thanksref{ai} \and
H.~M. Schutte\thanksref{z} \and
J.~Seneca\thanksref{t} \and
N.~Sennan\thanksref{aa} \and
B.~Setter\thanksref{ai} \and
I.~Sgura\thanksref{al} \and
R.~Shanidze\thanksref{au} \and
A.~Sharma\thanksref{o} \and
Y.~Shitov\thanksref{r} \and
F. \v{S}imkovic\thanksref{s} \and
A.~Simonelli\thanksref{f} \and
A.~Sinopoulou\thanksref{a} \and
M.V. Smirnov\thanksref{ai} \and
B.~Spisso\thanksref{f} \and
M.~Spurio\thanksref{v,u} \and
D.~Stavropoulos\thanksref{j} \and
I. \v{S}tekl\thanksref{r} \and
M.~Taiuti\thanksref{ap,p} \and
Y.~Tayalati\thanksref{n} \and
H.~Thiersen\thanksref{z} \and
I.~Tosta~e~Melo\thanksref{a,ak} \and
E.~Tragia\thanksref{j} \and
B.~Trocm{\'e}\thanksref{o} \and
V.~Tsourapis\thanksref{j} \and
A.Tudorache\thanksref{h,af} \and
E.~Tzamariudaki\thanksref{j} \and
A.~Vacheret\thanksref{q} \and
A.~Valer~Melchor\thanksref{t} \and
V.~Valsecchi\thanksref{y} \and
V.~Van~Elewyck\thanksref{aw,o} \and
G.~Vannoye\thanksref{c} \and
G.~Vasileiadis\thanksref{ba} \and
F.~Vazquez~de~Sola\thanksref{t} \and
C.~Verilhac\thanksref{o} \and
A. Veutro\thanksref{h,af} \and
S.~Viola\thanksref{y} \and
D.~Vivolo\thanksref{w,f} \and
J.~Wilms\thanksref{bb} \and
E.~de~Wolf\thanksref{ad,t} \and
H.~Yepes-Ramirez\thanksref{m} \and
G.~Zarpapis\thanksref{j} \and
S.~Zavatarelli\thanksref{p} \and
A.~Zegarelli\thanksref{h,af} \and
D.~Zito\thanksref{y} \and
J.\,D.~Zornoza\thanksref{e} \and
J.~Z{\'u}{\~n}iga\thanksref{e} \and
N.~Zywucka\thanksref{z} \\(KM3NeT Collaboration\thanksref{emailkm3}
}

\thankstext{e1}{e-mail: thijsvaneeden@gmail.com}
\thankstext{emailkm3}{e-mail: km3net-pc@km3net.de}

\institute{
\setlength{\parindent}{0pt}
INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 ~Italy\label{a} \and
Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France\label{b} \and
Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France\label{c} \and
University of Sharjah, Sharjah Academy for Astronomy, Space Sciences, and Technology, University Campus - POB 27272, Sharjah, - United Arab Emirates\label{d} \and
IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain\label{e} \and
INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy\label{f} \and
Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy\label{g} \and
INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy\label{h} \and
Universitat Polit{\`e}cnica de Catalunya, Laboratori d'Aplicacions Bioac{\'u}stiques, Centre Tecnol{\`o}gic de Vilanova i la Geltr{\'u}, Avda. Rambla Exposici{\'o}, s/n, Vilanova i la Geltr{\'u}, 08800 Spain\label{i} \and
NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece\label{j} \and
University of Granada, Dept.~of Computer Architecture and Technology/CITIC, 18071 Granada, Spain\label{k} \and
Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France\label{l} \and
Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain\label{m} \and
University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco\label{n} \and
Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France\label{o} \and
INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy\label{p} \and
LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France\label{q} \and
Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic\label{r} \and
Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic\label{s} \and
Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands\label{t} \and
INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy\label{u} \and
Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy\label{v} \and
Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy\label{w} \and
E.\,A.~Milne Centre for Astrophysics, University~of~Hull, Hull, HU6 7RX, United Kingdom\label{x} \and
INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy\label{y} \and
North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa\label{z} \and
University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco\label{aa} \and
Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy\label{ab} \and
ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania\label{ac} \and
University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands\label{ad} \and
TNO, Technical Sciences, PO Box 155, Delft, 2600 AD Netherlands\label{ae} \and
Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy\label{af} \and
Universit{\`a} di Bologna, Dipartimento di Ingegneria dell'Energia Elettrica e dell'Informazione "Guglielmo Marconi", Via dell'Universit{\`a} 50, Cesena, 47521 Italia\label{ag} \and
Cadi Ayyad University, Physics Department, Faculty of Science Semlalia, Av. My Abdellah, P.O.B. 2390, Marrakech, 40000 Morocco\label{ah} \and
Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany\label{ai} \and
University of the Witwatersrand, School of Physics, Private Bag 3, Johannesburg, Wits 2050 South Africa\label{aj} \and
Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy\label{ak} \and
INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy\label{al} \and
University W{\"u}rzburg, Emil-Fischer-Stra{\ss}e 31, W{\"u}rzburg, 97074 Germany\label{am} \and
Western Sydney University, School of Computing, Engineering and Mathematics, Locked Bag 1797, Penrith, NSW 2751 Australia\label{an} \and
IN2P3, LPC, Campus des C{\'e}zeaux 24, avenue des Landais BP 80026, Aubi{\`e}re Cedex, 63171 France\label{ao} \and
Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy\label{ap} \and
University of Granada, Dpto.~de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., 18071 Granada, Spain\label{aq} \and
NIOZ (Royal Netherlands Institute for Sea Research), PO Box 59, Den Burg, Texel, 1790 AB, the Netherlands\label{ar} \and
Leiden University, Leiden Institute of Physics, PO Box 9504, Leiden, 2300 RA Netherlands\label{as} \and
National~Centre~for~Nuclear~Research,~02-093~Warsaw,~Poland\label{at} \and
Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia\label{au} \and
The University of Georgia, Institute of Physics, Kostava str. 77, Tbilisi, 0171 Georgia\label{av} \and
Institut Universitaire de France, 1 rue Descartes, Paris, 75005 France\label{aw} \and
IN2P3, 3, Rue Michel-Ange, Paris 16, 75794 France\label{ax} \and
LPC, Campus des C{\'e}zeaux 24, avenue des Landais BP 80026, Aubi{\`e}re Cedex, 63171 France\label{ay} \and
University of Johannesburg, Department Physics, PO Box 524, Auckland Park, 2006 South Africa\label{az} \and
Laboratoire Univers et Particules de Montpellier, Place Eug{\`e}ne Bataillon - CC 72, Montpellier C{\'e}dex 05, 34095 France\label{ba} \and
Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Remeis Sternwarte, Sternwartstra{\ss}e 7, 96049 Bamberg, Germany\label{bb} \and
Universit{\'e} de Haute Alsace, rue des Fr{\`e}res Lumi{\`e}re, 68093 Mulhouse Cedex, France\label{bc} \and
AstroCeNT, Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, Rektorska 4, Warsaw, 00-614 Poland\label{bd}
}


==> frontpage.tex <==
\begin{frontmatter}

%% Title, authors and addresses

%% use the tnoteref command within \title for footnotes;
%% use the tnotetext command for theassociated footnote;
%% use the fnref command within \author or \address for footnotes;
%% use the fntext command for theassociated footnote;
%% use the corref command within \author for corresponding author footnotes;
%% use the cortext command for theassociated footnote;
%% use the ead command for the email address,
%% and the form \ead[url] for the home page:
%% \title{Title\tnoteref{label1}}
%% \tnotetext[label1]{}
%% \author{Name\corref{cor1}\fnref{label2}}
%% \ead{email address}
%% \ead[url]{home page}
%% \fntext[label2]{}
%% \cortext[cor1]{}
%% \address{Address\fnref{label3}}
%% \fntext[label3]{}

\title{Astronomy potential of KM3NeT/ARCA}

%% use optional labels to link authors explicitly to addresses:
% ----- Start automatically generated KM3NeT info
% ----- Start author list

\cortext[cor]{corresponding author}

\ead{km3net-pc@km3net.de}

\author[a]{S.~Aiello}
\author[b,bc]{A.~Albert}
\author[d,c]{M.~Alshamsi}
\author[e]{S. Alves Garre}
\author[c]{Z.~Aly}
\author[g,f]{A. Ambrosone}
\author[h]{F.~Ameli}
\author[i]{M.~Andre}
\author[j]{E.~Androutsou}
\author[k]{M.~Anguita}
\author[l]{L.~Aphecetche}
\author[m]{M. Ardid}
\author[m]{S. Ardid}
\author[n]{H.~Atmani}
\author[o]{J.~Aublin}
\author[p]{F.~Badaracco}
\author[q]{L.~Bailly-Salins}
\author[s,r]{Z. Barda\v{c}ov\'{a}}
\author[o]{B.~Baret}
\author[e]{A. Bariego-Quintana}
\author[p]{A.~Baruzzi}
\author[t]{S.~Basegmez~du~Pree}
\author[o]{Y.~Becherini}
\author[n,o]{M.~Bendahman}
\author[v,u]{F.~Benfenati}
\author[w,f]{M.~Benhassi}
\author[x]{D.\,M.~Benoit}
\author[t]{E.~Berbee}
\author[c]{V.~Bertin}
\author[y]{S.~Biagi}
\author[z]{M.~Boettcher}
\author[y]{D.~Bonanno}
\author[n]{J.~Boumaaza}
\author[aa]{M.~Bouta}
\author[t]{M.~Bouwhuis}
\author[ab,f]{C.~Bozza}
\author[g,f]{R.\,M.~Bozza}
\author[ac]{H.Br\^{a}nza\c{s}}
\author[l]{F.~Bretaudeau}
\author[c]{M.~Breuhaus}
\author[ad,t]{R.~Bruijn}
\author[c]{J.~Brunner}
\author[a]{R.~Bruno}
\author[ae,t]{E.~Buis}
\author[w,f]{R.~Buompane}
\author[c]{J.~Busto}
\author[p]{B.~Caiffi}
\author[e]{D.~Calvo}
\author[h,af]{S.~Campion}
\author[h,af]{A.~Capone}
\author[v,u]{F.~Carenini}
\author[e]{V.~Carretero}
\author[o]{T.~Cartraud}
\author[ag,u]{P.~Castaldi}
\author[e]{V.~Cecchini}
\author[h,af]{S.~Celli}
\author[c]{L.~Cerisy}
\author[ah]{M.~Chabab}
\author[ai]{M.~Chadolias}
\author[aj]{A.~Chen}
\author[ak,y]{S.~Cherubini}
\author[u]{T.~Chiarusi}
\author[al]{M.~Circella}
\author[y]{R.~Cocimano}
\author[o]{J.\,A.\,B.~Coelho}
\author[o]{A.~Coleiro}
\author[y]{R.~Coniglione}
\author[c]{P.~Coyle}
\author[o]{A.~Creusot}
\author[y]{G.~Cuttone}
\author[l]{R.~Dallier}
\author[ai]{Y.~Darras}
\author[f]{A.~De~Benedittis}
\author[c]{B.~De~Martino}
\author[l]{V.~Decoene}
\author[f]{R.~Del~Burgo}
\author[v,u]{I.~Del~Rosso}
\author[y]{L.\,S.~Di~Mauro}
\author[h,af]{I.~Di~Palma}
\author[k]{A.\,F.~D\'\i{}az}
\author[k]{C.~Diaz}
\author[y]{D.~Diego-Tortosa}
\author[y]{C.~Distefano}
\author[ai]{A.~Domi}
\author[o]{C.~Donzaud}
\author[c]{D.~Dornic}
\author[am]{M.~D{\"o}rr}
\author[j]{E.~Drakopoulou}
\author[b,bc]{D.~Drouhin}
\author[c]{J.-G. Ducoin}
\author[s]{R. Dvornick\'{y}}
\author[ai]{T.~Eberl}
\author[s,r]{E. Eckerov\'{a}}
\author[n]{A.~Eddymaoui}
\author[t]{T.~van~Eeden\corref{cor}}
\ead{tjuanve@nikhef.nl}
\author[o]{M.~Eff}
\author[t]{D.~van~Eijk}
\author[aa]{I.~El~Bojaddaini}
\author[o]{S.~El~Hedri}
\author[c]{A.~Enzenh\"ofer}
\author[y]{G.~Ferrara}
\author[an]{M.~D.~Filipovi\'c}
\author[v,u]{F.~Filippini}
\author[y]{D.~Franciotti}
\author[ab,f]{L.\,A.~Fusco}
\author[ao]{J.~Gabriel}
\author[h]{S.~Gagliardini}
\author[ai]{T.~Gal}
\author[m]{J.~Garc{\'\i}a~M{\'e}ndez}
\author[e]{A.~Garcia~Soto}
\author[t]{C.~Gatius~Oliver}
\author[ai]{N.~Gei{\ss}elbrecht}
\author[aa]{H.~Ghaddari}
\author[f,w]{L.~Gialanella}
\author[x]{B.\,K.~Gibson}
\author[y]{E.~Giorgio}
\author[o]{I.~Goos}
\author[o]{P.~Goswami}
\author[q]{D.~Goupilliere}
\author[e]{S.\,R.~Gozzini}
\author[ai]{R.~Gracia}
\author[ai]{K.~Graf}
\author[ap,p]{C.~Guidi}
\author[q]{B.~Guillon}
\author[aq]{M.~Guti{\'e}rrez}
\author[ar]{H.~van~Haren}
\author[t]{A.~Heijboer}
\author[am]{A.~Hekalo}
\author[ai]{L.~Hennig}
\author[e]{J.\,J.~Hern{\'a}ndez-Rey}
\author[f]{W.~Idrissi~Ibnsalih}
\author[u]{G.~Illuminati}
\author[as,t]{M.~de~Jong}
\author[ad,t]{P.~de~Jong}
\author[t]{B.\,J.~Jung}
\author[at,bd]{P.~Kalaczy\'nski}
\author[ai]{O.~Kalekin}
\author[ai]{U.\,F.~Katz}
\author[s]{A.~Khatun}
\author[av,au]{G.~Kistauri}
\author[ai]{C.~Kopper}
\author[aw,o]{A.~Kouchner}
\author[t]{V.~Kueviakoe}
\author[p]{V.~Kulikovskiy}
\author[av]{R.~Kvatadze}
\author[q]{M.~Labalme}
\author[ai]{R.~Lahmann}
\author[y]{G.~Larosa}
\author[c]{C.~Lastoria}
\author[e]{A.~Lazo}
\author[c]{S.~Le~Stum}
\author[q]{G.~Lehaut}
\author[a]{E.~Leonora}
\author[e]{N.~Lessing}
\author[v,u]{G.~Levi}
\author[o]{M.~Lindsey~Clark}
\author[a]{F.~Longhitano}
\author[c]{F.~Magnani}
\author[t]{J.~Majumdar}
\author[p]{L.~Malerba}
\author[r]{F.~Mamedov}
\author[e]{J.~Ma\'nczak}
\author[f]{A.~Manfreda}
\author[ap,p]{M.~Marconi}
\author[v,u]{A.~Margiotta}
\author[f,g]{A.~Marinelli}
\author[j]{C.~Markou}
\author[l]{L.~Martin}
\author[m]{J.\,A.~Mart{\'\i}nez-Mora}
\author[w,f]{F.~Marzaioli}
\author[af,h]{M.~Mastrodicasa}
\author[f]{S.~Mastroianni}
\author[y]{S.~Miccich{\`e}}
\author[g,f]{G.~Miele}
\author[f]{P.~Migliozzi}
\author[y]{E.~Migneco}
\author[f]{M.\,L.~Mitsou}
\author[f]{C.\,M.~Mollo}
\author[w,f]{L. Morales-Gallegos}
\author[al]{M.~Morga}
\author[aa]{A.~Moussa}
\author[ay,ax]{I.~Mozun~Mateo}
\author[t]{R.~Muller}
\author[f,w]{M.\,R.~Musone}
\author[y]{M.~Musumeci}
\author[aq]{S.~Navas}
\author[al]{A.~Nayerhoda}
\author[h]{C.\,A.~Nicolau}
\author[aj]{B.~Nkosi}
\author[ad,t]{B.~{\'O}~Fearraigh}
\author[g,f]{V.~Oliviero}
\author[y]{A.~Orlando}
\author[o]{E.~Oukacha}
\author[y]{D.~Paesani}
\author[e]{J.~Palacios~Gonz{\'a}lez}
\author[al,au]{G.~Papalashvili}
\author[ap,p]{V.~Parisi}
\author[e]{E.J. Pastor Gomez}
\author[ac]{A.~M.~P{\u a}un}
\author[ac]{G.\,E.~P\u{a}v\u{a}la\c{s}}
\author[j]{I.~Pelegris}
\author[o]{S. Pe\~{n}a Mart\'inez}
\author[c]{M.~Perrin-Terrin}
\author[q]{J.~Perronnel}
\author[ay]{V.~Pestel}
\author[o]{R.~Pestes}
\author[y]{P.~Piattelli}
\author[ab,f]{C.~Poir{\`e}}
\author[ac]{V.~Popa}
\author[b]{T.~Pradier}
\author[e]{J.~Prado}
\author[y]{S.~Pulvirenti}
\author[m]{C.A.~Quiroz-Rangel}
\author[e]{U.~Rahaman}
\author[a]{N.~Randazzo}
\author[l]{R.~Randriatoamanana}
\author[az]{S.~Razzaque}
\author[f]{I.\,C.~Rea}
\author[e]{D.~Real}
\author[y]{G.~Riccobene}
\author[z]{J.~Robinson}
\author[ap,p]{A.~Romanov}
\author[e]{A. \v{S}aina}
\author[e]{F.~Salesa~Greus}
\author[as,t]{D.\,F.\,E.~Samtleben}
\author[e,al]{A.~S{\'a}nchez~Losa}
\author[y]{S.~Sanfilippo}
\author[ap,p]{M.~Sanguineti}
\author[w,f]{C.~Santonastaso}
\author[y]{D.~Santonocito}
\author[y]{P.~Sapienza}
\author[ai]{J.~Schnabel}
\author[ai]{J.~Schumann}
\author[z]{H.~M. Schutte}
\author[t]{J.~Seneca}
\author[aa]{N.~Sennan}
\author[ai]{B.~Setter}
\author[al]{I.~Sgura}
\author[au]{R.~Shanidze}
\author[o]{A.~Sharma}
\author[r]{Y.~Shitov}
\author[s]{F. \v{S}imkovic}
\author[f]{A.~Simonelli}
\author[a]{A.~Sinopoulou}
\author[ai]{M.V. Smirnov}
\author[f]{B.~Spisso}
\author[v,u]{M.~Spurio}
\author[j]{D.~Stavropoulos}
\author[r]{I. \v{S}tekl}
\author[ap,p]{M.~Taiuti}
\author[n]{Y.~Tayalati}
\author[z]{H.~Thiersen}
\author[a,ak]{I.~Tosta~e~Melo}
\author[j]{E.~Tragia}
\author[o]{B.~Trocm{\'e}}
\author[j]{V.~Tsourapis}
\author[h,af]{A.Tudorache}
\author[j]{E.~Tzamariudaki}
\author[q]{A.~Vacheret}
\author[t]{A.~Valer~Melchor}
\author[y]{V.~Valsecchi}
\author[aw,o]{V.~Van~Elewyck}
\author[c]{G.~Vannoye}
\author[ba]{G.~Vasileiadis}
\author[t]{F.~Vazquez~de~Sola}
\author[o]{C.~Verilhac}
\author[h,af]{A. Veutro}
\author[y]{S.~Viola}
\author[w,f]{D.~Vivolo}
\author[bb]{J.~Wilms}
\author[ad,t]{E.~de~Wolf}
\author[m]{H.~Yepes-Ramirez}
\author[j]{G.~Zarpapis}
\author[p]{S.~Zavatarelli}
\author[h,af]{A.~Zegarelli}
\author[y]{D.~Zito}
\author[e]{J.\,D.~Zornoza}
\author[e]{J.~Z{\'u}{\~n}iga}
\author[z]{N.~Zywucka}
% ----- End author list
% ----- Start address list
\address[a]{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\address[b]{Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France}
\address[c]{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\address[d]{University of Sharjah, Sharjah Academy for Astronomy, Space Sciences, and Technology, University Campus - POB 27272, Sharjah, - United Arab Emirates}
\address[e]{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\address[f]{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\address[g]{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\address[h]{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\address[i]{Universitat Polit{\`e}cnica de Catalunya, Laboratori d'Aplicacions Bioac{\'u}stiques, Centre Tecnol{\`o}gic de Vilanova i la Geltr{\'u}, Avda. Rambla Exposici{\'o}, s/n, Vilanova i la Geltr{\'u}, 08800 Spain}
\address[j]{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\address[k]{University of Granada, Dept.~of Computer Architecture and Technology/CITIC, 18071 Granada, Spain}
\address[l]{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\address[m]{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\address[n]{University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco}
\address[o]{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\address[p]{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\address[q]{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\address[r]{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\address[s]{Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic}
\address[t]{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\address[u]{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\address[v]{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\address[w]{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\address[x]{E.\,A.~Milne Centre for Astrophysics, University~of~Hull, Hull, HU6 7RX, United Kingdom}
\address[y]{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\address[z]{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\address[aa]{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\address[ab]{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\address[ac]{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\address[ad]{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\address[ae]{TNO, Technical Sciences, PO Box 155, Delft, 2600 AD Netherlands}
\address[af]{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\address[ag]{Universit{\`a} di Bologna, Dipartimento di Ingegneria dell'Energia Elettrica e dell'Informazione "Guglielmo Marconi", Via dell'Universit{\`a} 50, Cesena, 47521 Italia}
\address[ah]{Cadi Ayyad University, Physics Department, Faculty of Science Semlalia, Av. My Abdellah, P.O.B. 2390, Marrakech, 40000 Morocco}
\address[ai]{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\address[aj]{University of the Witwatersrand, School of Physics, Private Bag 3, Johannesburg, Wits 2050 South Africa}
\address[ak]{Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\address[al]{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\address[am]{University W{\"u}rzburg, Emil-Fischer-Stra{\ss}e 31, W{\"u}rzburg, 97074 Germany}
\address[an]{Western Sydney University, School of Computing, Engineering and Mathematics, Locked Bag 1797, Penrith, NSW 2751 Australia}
\address[ao]{IN2P3, LPC, Campus des C{\'e}zeaux 24, avenue des Landais BP 80026, Aubi{\`e}re Cedex, 63171 France}
\address[ap]{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\address[aq]{University of Granada, Dpto.~de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., 18071 Granada, Spain}
\address[ar]{NIOZ (Royal Netherlands Institute for Sea Research), PO Box 59, Den Burg, Texel, 1790 AB, the Netherlands}
\address[as]{Leiden University, Leiden Institute of Physics, PO Box 9504, Leiden, 2300 RA Netherlands}
\address[at]{National~Centre~for~Nuclear~Research,~02-093~Warsaw,~Poland}
\address[au]{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\address[av]{The University of Georgia, Institute of Physics, Kostava str. 77, Tbilisi, 0171 Georgia}
\address[aw]{Institut Universitaire de France, 1 rue Descartes, Paris, 75005 France}
\address[ax]{IN2P3, 3, Rue Michel-Ange, Paris 16, 75794 France}
\address[ay]{LPC, Campus des C{\'e}zeaux 24, avenue des Landais BP 80026, Aubi{\`e}re Cedex, 63171 France}
\address[az]{University of Johannesburg, Department Physics, PO Box 524, Auckland Park, 2006 South Africa}
\address[ba]{Laboratoire Univers et Particules de Montpellier, Place Eug{\`e}ne Bataillon - CC 72, Montpellier C{\'e}dex 05, 34095 France}
\address[bb]{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Remeis Sternwarte, Sternwartstra{\ss}e 7, 96049 Bamberg, Germany}
\address[bc]{Universit{\'e} de Haute Alsace, rue des Fr{\`e}res Lumi{\`e}re, 68093 Mulhouse Cedex, France}
\address[bd]{AstroCeNT, Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, Rektorska 4, Warsaw, 00-614 Poland}
% ----- End address list
% ----- End automatically generated KM3NeT info

\newpage

\begin{abstract}
The KM3NeT/ARCA neutrino detector is currently under construction at 3500 m depth offshore Capo Passero, Sicily, in the Mediterranean Sea. The main science objectives are the detection of high-energy cosmic neutrinos and the discovery of their sources. Simulations were conducted for the full KM3NeT/ARCA detector, instrumenting a volume of 1 km$^3$, to estimate the sensitivity and discovery potential to point-like neutrino sources and an all-sky diffuse neutrino flux. This paper covers the reconstruction of track- and shower-like signatures, as well as the criteria employed for neutrino event selection. By leveraging both the track and shower observation channels, the KM3NeT/ARCA detector demonstrates the capability to detect the diffuse astrophysical neutrino flux within half a year of operation, achieving a 5$\sigma$ statistical significance. With an angular resolution below 0.1$^\circ$ for tracks and under 2$^\circ$ for showers, the sensitivity to point-like neutrino sources surpasses existing observed limits across the entire sky.
\end{abstract}

\end{frontmatter}

